A little goes a long way: Improving toxic language classification despite data scarcity

Detection of some types of toxic language is hampered by extreme scarcity of labeled training data. Data augmentation - generating new synthetic data from a labeled seed dataset - can help. The efficacy of data augmentation on toxic language classification has not been fully explored. We present the first systematic study on how data augmentation techniques impact performance across toxic language classifiers, ranging from shallow logistic regression architectures to BERT - a state-of-the-art pre-trained Transformer network. We compare the performance of eight techniques on very scarce seed datasets. We show that while BERT performed the best, shallow classifiers performed comparably when trained on data augmented with a combination of three techniques, including GPT-2-generated sentences. We discuss the interplay of performance and computational overhead, which can inform the choice of techniques under different constraints.

==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We compared several techniques for increasing toxicity classification performance
by data augmentation, in scenarios with
very scarce labeled toxic documents. 
Our results highlight that while \bert~with simple oversampling performs remarkably well,
simpler classifiers like character-based logistic regression can perform \myemph{on par} with \bert, provided that appropriate data augmentation is applied to the training set. 
By contrast, we found that \bert~results were difficult to improve beyond simple oversampling. 
%in datasets with
%very scarce labeled offensive documents. 
% synthetically increasing the number of toxic documents in very 

==> sections/scratch.tex <==
% Here are some of the "safer" threats
% If you block me for telling you what you are, there will bw a holy war, I promise you that. (row 1156, 0312.txt)
% if you do not stop, the wikapidea nijas will come to your house and kill you (row 5063)
%     Chipmunk Can you please stop vandalising the Chipmunk. if you do not stop, the wikapidea nijas will come to your house and kill you
%   We thank you both for your contributions to Wikipedia at-large and your use of the tool. if you do not stop, the wikapidea nijas will come to your house and kill you
% I am going to kill you I am going to murder you (row 8042)
% I am going to kill you I am going to murder you And if you have any more questions after that, feel free to post them on my user talk page or place {{helpme}} on your talk page and someone will be by to help you shortly.
% I'll attack you! 32.210.212.23 (976, 0311.txt)
% The only objection is from the creator of the article. Insult me once more and I swear you go down. Understand little coward? (row 3566)
% I really hate you And I want to do nasty things to you (row 7126)
% I'm sure that both violations were inadvertent, and that you'll either comply or seek to change the policy. I really hate you And I want to do nasty things to you
% Wtf, Why You deleting Maashel? Bad things will happen to you now. (row 6817, 0310.txt)
% Wtf, Why You deleting Maashel? I didn't do anything wrong... Bad things will happen to you now.
% I am going to kill you. I am going to murder you. (row 7477)
% Got the note... I am going to kill you. I am going to murder you.

%if you do put up not stop the wikapidea nijas will come to your house and kill you
\begin{table*}[tbh]
  \begin{center}
    \begin{tabular}{ll}
    \hline
     & Document sample \\
    \hline
    \tikzmark{a}\seed
         & if you do not stop, the wikapidea 
         %\\  & 
         nijas will come to your house
         %\\ & 
         and kill you \\
    \tikzmark{x0}~~~\tikzmark{x}\simple 
         & if you do not stop, the wikapidea 
         %\\  & 
         nijas will come to your house
         %\\ & 
         and kill you \\
    \tikzmark{e0}~~~\tikzmark{e}\eda  
    & if you do \textit{put up} not stop the 
         %\\  & 
         wikapidea nijas will come to 
         %\\  & 
         your house and kill you \\    
    %\hline         
    \tikzmark{b0}~~~\tikzmark{b}\add 
        & \textit{We thank you both for your} 
         %\\  & 
         \textit{contributions to Wikipedia at-large} 
         %\\  & 
         \textit{and your use of the tool.} \\
         & if you 
         %\\  & 
         do not stop, the wikapidea nijas will 
         %\\  & 
         come to your house and kill you \\
% if you do not be halted , the wikapidea nijas will come to your home and kill you
    \tikzmark{g0}~~~\tikzmark{g}\ppdb
%         &     \begin{tabular}{l}
%         if you do not \textit{be halted} , the wikapidea
%         nijas will come to your \textit{home} 
%         and kill you \\         
%         \end{tabular} \\
         & if you do not \textit{be halted} , the wikapidea 
         %\\  & 
         nijas will come to your \textit{home} 
         %\\  & 
         and kill you \\         
% if you do not stop , the wikapidea nijas will amount to your house and kill you
    \tikzmark{h0}~~~\tikzmark{h}\wn
         & if you do not stop , the wikapidea 
         %\\  & 
         nijas will \textit{amount} to your house 
         %\\  & 
         and kill you \\       
    %if you so not stop , the wikapidea nijas will come to yours house have kill you
    \tikzmark{f0}~~~\tikzmark{f}\gensim
         & if you \textit{so} not stop , the wikapidea 
         %\\  & 
         nijas will come to your\textit{s} house 
         %\\  & 
         \textit{have} kill you \\
    \tikzmark{c0}~~~\tikzmark{c}\bpemb 
    & \textit{whether} you \textit{know} not stop,  
         %\\  & 
         the\textit{ldi}kapide\textit{ina} ni\textit{ji} \textit{give} 
         %\\  & 
         come to your house and kill you \\
    \tikzmark{d0}~~~\tikzmark{d}\gpt
    & \textit{for what you have done, you don't} 
         %\\  & 
         \textit{have a choice. You are too big and} 
         %\\  & 
         \textit{weak to stop.}\\
    \hline         
    \end{tabular}
    \caption{Documents generated by selected methods in this study. Changes to original seed \textit{highlighted}. % with \textit{italics.
    The selected  sample is shorter than average (see Table~\ref{tab:data-stats}). }
    \label{tab:example}
  \end{center}
\end{table*}


\iffalse
\begin{table*}[!h]
  \begin{center}
    \begin{tabular}{llccccc}
    \hline
    \multirow{2}{*}{\textbf{Classifier}}& \multirow{2}{*}{\textbf{Metric}}& \multicolumn{5}{c}{\textbf{Neighborhood size $k$}} \\
    %\hline
     &&1&3&5&7&10 \\ %&8&9&10\\
     \hline
    \multirow{3}{*}{char-lr}&precision & \textbf{0.59} & 0.58 & 0.57 & 0.57 & 0.56 \\
    &recall & \textbf{0.22} & \textbf{0.22} & \textbf{0.22} & \textbf{0.22} & \textbf{0.22} \\
    &F1 (macro) & \textbf{0.66} & \textbf{0.66} & \textbf{0.66} & \textbf{0.66} & 0.65 \\
    \hline
    \multirow{3}{*}{word-lr}&precision & \textbf{0.34} & \textbf{0.34} & \textbf{0.34} & \textbf{0.34} & \textbf{0.34} \\
    &recall & 0.21 & \textbf{0.22} & \textbf{0.22} & \textbf{0.22} & 0.21 \\
    &F1 (macro) & \textbf{0.63} & \textbf{0.63} & \textbf{0.63} & \textbf{0.63} & \textbf{0.63} \\
    \hline
    \multirow{3}{*}{cnn}&precision & \textbf{0.32} & 0.31 & 0.27 & 0.28 & 0.25 \\
    &recall & 0.33 & 0.35 & 0.36 & \textbf{0.37} & 0.36 \\
    &F1 (macro) & \textbf{0.66} & \textbf{0.63} & 0.65 & 0.65 & 0.64 \\
    \hline
    \multirow{3}{*}{bert}&precision & 0.37 & 0.37 & 0.37 & \textbf{0.38} & \textbf{0.38} \\
    &recall & \textbf{0.18} & 0.16 & 0.16 & 0.17 & 0.16 \\
    &F1 (macro) & \textbf{0.61} & \textbf{0.61} & \textbf{0.61} & \textbf{0.61} & \textbf{0.61} \\
    \hline   
    \end{tabular}
    \caption{Impact of choosing between different number of top-candidates $k$ in \bpemb-augmented datasets. Mean results for 10 repetitions. Highest numbers highlighted in bold. }
    \label{tab:bpemb-change-rate}
  \end{center}
\end{table*}    
\fi


\begin{algorithmic}
\STATE{1.} $m \gets$ specify a metric
\STATE{2.} $c \gets$ Specify a classifier
\STATE{3.} Calculate mean metric value for 
\FORALL{augmentation techniques $a_\textrm{i} \in A$} 
    \FORALL{random \seed $s_j \in S$} 
        \STATE{\textbf{train} $c_j$ on $s_j$} 
        \STATE{\textbf{calculate} metric $m_{ij} \gets$ $m_i(c_j$,\test)} 
    \ENDFOR
    \STATE{$\hat{m}_{i} \gets$ mean($m_{ij}$)}
\ENDFOR
\STATE{$i* \gets \textrm{argmax}(\hat{m}_i)$}
\FORALL{augmentation techniques $a_\textrm{i} \in A$} 
    \FORALL{random \seed $s_j \in S$} 
        \STATE{\textbf{calculate} difference $d_{ij} \gets m_{i*j} - m_{ij}$}
        \STATE $v \gets \textrm{Var}(d_{ij})$
        \STATE $d \gets \textrm{mean}(d_{ij})$
        \STATE $n \gets \textrm{sqrt}(v / |S|)$
        \STATE $t \gets d / n$
        \STATE $p \gets \textrm{table}(t)$
        \STATE $p \gets p/2$ // one-tailed test
    \ENDFOR
\ENDFOR
\end{algorithmic}

%We apply the algorithm 

==> sections/statistics.tex <==
\section{Statistical tests}
\label{app:stats}

We supply additional information on statistical tests performed in this study. 
For each statistical test, we compared 30 numbers from two paired experimental setup ($a$ vs. $b$), e.g. (Precision of \charlr on \simple vs \eda). 

\iffalse
We calculated our test statistic as: 
%and annotate statistically significant differences in tables the following way:
\begin{equation}
    t = \dfrac{\bar{x}}{s_D \sqrt{n}}, 
\end{equation}
where $n=30$ is the number of repetitions, $\bar{x}$ is the mean of $n$ differences in the number between setups $a$ and $b$, $s_D$ is the standard deviation of this difference. 

The one-tailed t-test describes whether one measure $a$ is statistically larger than the other $b$. In our tests, $a$ always represents the highest value for a combination of metric and classifier. We calculated this probability with $n-1$ degrees of freedom.~\cite{murphy2012machine} 
%Paired t-test functionality is provided by scipy \footnote{\url{https://docs.scipy.org/doc/scipy/reference/generated/scipy.stats.ttest_rel.html}}.
\fi

In Tables~\ref{tab:results-augmentations-statistics} -- \ref{tab:roc_auc} (\S\ref{sec:augmentations} -- \S\ref{sec:tradeoff}) we give indication of statistical significance with double underlines and bolding. 
Actual p-values are described in Tables~\ref{tab:results-augmentations-statistics} -- 
Table~\ref{tab:results-combination-statistics}.

\begin{table}[!h]
  \begin{center}
    \begin{tabular}{lllll}
    \hline
    & \multicolumn{4}{c}{Macro-averaged F1-score} \\
     Augmentation & \charlrshort & \wordlrshort & \cnn & \bert \\
    \hline
    \seed   & 5e-31 & 2e-27 & 3e-15 & 2e-35 \\
    \simple & 9e-15 & 7e-26 & 2e-23 & \textbf{8e-2} \\
    \eda    & 2e-17 & 2e-21 & 2e-22 & 9e-31 \\
    \add    & 2e-3  & 7e-22 & 4e-7  & * \\
    \ppdb   & 2e-25 & 6e-26 & 3e-20 & 6e-3 \\
    \wn     & 3e-26 & 5e-25 & 8e-18 & 8e-7 \\
    \gensim & 3e-25 & 3e-15 & 6e-10 & 3e-15 \\
    \bpemb  & 8e-7  & 3e-16 & 3e-6  & 1e-16 \\
    \gpt    & * & * & * & 2e-16 \\
    \hline
    \hline
    & \multicolumn{4}{c}{\cls{threat} precision} \\
     Augmentation & \charlrshort & \wordlrshort & \cnn &    \bert \\
     \hline
    \seed & * & * & * & 4e-27\\
    \simple & \textbf{5e-1} & \textbf{8e-2} & 4e-2 & * \\
    \eda & \textbf{4e-1} & 2e-2 & 3e-7 & 2e-21\\
    \add  & 6e-3 & 8e-3 & \textbf{5e-1} & 4e-13\\
    \ppdb & 3e-14 & \textbf{3e-1} & 2e-3 & \textbf{2e-2}\\
    \wn & 2e-14 & 3e-2 & \textbf{7e-2} & 4e-2\\
    \gensim & 2e-14 & \textbf{2e-1} & 8e-3 & 2e-4\\
    \bpemb & 3e-3 & 2e-2 & 2e-9 & 7e-8\\
    \gpt & 5e-7 & 4e-2 & 4e-5 & 3e-23\\     
    \hline
    \hline
    & \multicolumn{4}{c}{\cls{threat} recall} \\
     Augmentation & \charlrshort & \wordlrshort & \cnn &   \bert \\ 
     \hline
    \seed   & 2e-27 & 2e-27 & 9e-19  & 2e-26 \\
    \simple & 2e-17 & 2e-28 & 1e-18 & 7e-18 \\
    \eda    & 2e-19 & 9e-24 & 2e-19 & 2e-25 \\
    \add    & 2e-8  & 4e-26 & 2e-13 & 5e-7  \\
    \ppdb   & 2e-22  & 9e-28 & 2e-18 & 2e-18 \\
    \wn     & 3e-21 & 2e-25 & 4e-17 & 9e-21 \\
    \gensim & 2e-20 & 9e-19 & 2e-14 & 3e-20 \\
    \bpemb  & 2e-11 & 9e-17 & 1e-4  & 2e-22 \\
    \gpt    & * & * & * & *\\     
    \hline
    \end{tabular}
    \caption{p-values for statistical tests performed in Table~\ref{tab:results-augmented}. Tests are performed in each column, for each performance metric. The best-performing augmentation is denoted with asterisk (*). A one-tailed t-tests for related pairs is performed with regard to this point of reference. Rounded up (one significant digit). Statistically insignificant differences bolded (significance level $\alpha = $5e-2.) }
    \label{tab:results-augmentations-statistics}
  \end{center}
\end{table}

\begin{table}[!h]
  \begin{center}
    \begin{tabular}{lllll}
    \hline
    & \multicolumn{4}{c}{Macro-averaged F1-score} \\
     Augmentation & \charlrshort & \wordlrshort & \cnn & \bert \\
    \hline
    \seed   & 4e-32 & 4e-27 & 4e-16 & 2e-35 \\
    \simple & 5e-21 & 7e-27 & 5e-22 & \textbf{8e-2} \\
    \eda    & 4e-22 & 8e-22 & 6e-25 & 9e-31 \\
    \add    & 5e-11 & 2e-26 & 2e-8  & * \\
    \ppdb   & 2e-28 & 2e-25 & 1e-20 & 6e-3 \\
    \wn     & 6e-30 & 3e-25 & 2e-17 & 8e-7 \\
    \gensim & 6e-30 & 2e-15 & 3e-12 & 3e-15 \\
    \bpemb  & 5e-15 & 6e-16 & 2e-11  & 1e-16 \\
    \gpt    & 3e-7  & \textbf{4e-1} & 7e-4 & 2e-16 \\
    \ab     & 8e-11 & 5e-17 & 2e-3 & 2e-4 \\
    \abg    & * & * & * & 2e-4 \\    
    \hline
    \hline
    & \multicolumn{4}{c}{\cls{threat} precision} \\
     Augmentation & \charlrshort & \wordlrshort & \cnn &    \bert \\
     \hline
    \seed & * & * & * & 4e-27\\
    \simple & \textbf{5e-1} & \textbf{8e-2} & 4e-2 & * \\
    \eda & \textbf{4e-1} & 2e-2 & 3e-7 & 2e-21\\
    \add  & 6e-3 & 8e-3 & \textbf{5e-1} & 4e-13\\
    \ppdb & 3e-14 & \textbf{3e-1} & 2e-3 & \textbf{2e-2}\\
    \wn & 2e-14 & 3e-2 & \textbf{7e-2} & 4e-2\\
    \gensim & 2e-14 & \textbf{2e-1} & 8e-3 & 2e-4\\
    \bpemb & 3e-3 & 2e-2 & 2e-9 & 7e-8\\
    \gpt & 5e-7 & 4e-2 & 4e-5 & 3e-23\\     
    \ab     & 1e-3 & 5e-2 & 5e-5 & 4e-9 \\
    \abg    & 3e-6 & \textbf{1e-1} & 4e-5 & 1e-18 \\      
    \hline
    \hline
    & \multicolumn{4}{c}{\cls{threat} recall} \\
     Augmentation & \charlrshort & \wordlrshort & \cnn &   \bert \\ 
     \hline
% baseline 1.739239e-29
%***
% copy 5.255156e-20
%***
% eda 1.433600e-28
%***
% add 1.793531e-12
%***
% ppdb-c25 1.550152e-19
%***
% wn-c25 2.704678e-22
%***
% gensim-c25-s00 9.396965e-23
%***
% bpemb-c25-s00 1.533913e-24
%***
% gpt2-epoch2 2.438305e-02
%**
% add_bpemb-c25-s00 8.378033e-18
%***
    \seed   & 8e-30 & 2e-27 & 9e-23  & 2e-29 \\
    \simple & 7e-23 & 2e-28 & 2e-24 & 6e-20 \\
    \eda    & 6e-24 & 9e-24 & 2e-24 & 2e-28 \\
    \add    & 2e-14  & 4e-26 & 2e-19 & 2e-12  \\
    \ppdb   & 2e-26  & 9e-28 & 6e-24 & 2e-19 \\
    \wn     & 8e-25 & 2e-25 & 6e-22 & 3e-22 \\
    \gensim & 7e-26 & 9e-19 & 4e-19 & 1e-22 \\
    \bpemb  & 4e-18 & 9e-17 & 3e-11 & 2e-24 \\
    \gpt    & 2e-5  & * & 3e-5 & 3e-2\\   
    \ab     & 2e-14 & 9e-19 & 9e-10 & 9e-19 \\
    \abg    & * & 2e-6 & * & * \\      
    \hline
    \end{tabular}
    \caption{p-values for statistical tests performed in Table~\ref{tab:results-combinations}. Tests are performed in each column, for each performance metric. The best-performing augmentation is denoted with asterisk (*). A one-tailed t-tests for related pairs is performed with regard to this point of reference. Rounded up (one significant digit). Statistically insignificant differences bolded (significance level $\alpha = $5e-2.) }
    \label{tab:results-combination-statistics}
  \end{center}
\end{table}


